Simulating the weak death of the neutron in a femtoscale universe with near-Exascale computing

The fundamental particle theory called Quantum Chromodynamics (QCD) dictates everything about protons and neutrons, from their intrinsic properties to interactions that bind them into atomic nuclei. Quantities that cannot be fully resolved through experiment, such as the neutron lifetime (whose precise value is important for the existence of light-atomic elements that make the sun shine and life possible), may be understood through numerical solutions to QCD. We directly solve QCD using Lattice Gauge Theory and calculate nuclear observables such as neutron lifetime. We have developed an improved algorithm that exponentially decreases the time-to solution and applied it on the new CORAL supercomputers, Sierra and Summit. We use run-time autotuning to distribute GPU resources, achieving 20% performance at low node count. We also developed optimal application mapping through a job manager, which allows CPU and GPU jobs to be interleaved, yielding 15% of peak performance when deployed across large fractions of CORAL.

==> macros.tex <==
\usepackage{xspace}
\usepackage{bbm}

%%%%
%%%%    Referring to Parts of the Document
%%%%

\newcommand{\tabref}[1]{Tab.~\ref{tab:#1}\xspace}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}\xspace}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}\xspace}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}\xspace}
\renewcommand{\eqref}[1]{(\ref{#1})\xspace}
\newcommand{\Eqref}[1]{Equation~\ref{eq:#1}\xspace}

%%%%
%%%%    Mathematical Symbols
%%%%

\newcommand{\goesto}{\ensuremath{\rightarrow}}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}

%%%%
%%%%    Physical Quantities and Constants
%%%%


%%%%
%%%%    Software
%%%%

\newcommand{\git}{\texttt{git}\xspace}

% Put an xspace after \LaTeX:
\let\builtinLaTeX\LaTeX
\def\LaTeX{\builtinLaTeX\xspace}


==> section/implications.tex <==
\section{\label{sec:impl_results} Implications}

The trend shown in Table \ref{tab:systems} is representative of
high-performance computing in general: that being that nodes are
becoming denser, whether literally in the sense of increasing numbers
of accelerators per node, or virtually in the sense that local compute
is increasing generation to generation faster than the interconncet
bandwidth.  For example, if we compare Sierra and Titan, we see a
\(\sim 35\times\)
increase in flops per node, compared to only a \(\sim 3\times\)
increase in network bandwidth per node.  For task-parallel problems, such as the
LQCD problem at hand, this can represent an impasse with respect to
their ability to utilize next-generation machines (and the Exascale
beyond that).  Innovation in software and algorithms is critical to
enable these machines to be fully utilized, since the usual data
parallelism domain decomposition approaches will no longer suffice.

Of course, high-performance GPU-capable software such as QUDA goes a long way to extracting useful work from these machines.  But without an easy way to manage tasks and overlay independent work, these task-parallel problems will struggle to take advantage of the full capability of the dense architecture.  Our job manager, \texttt{mpi\_jm}, will make it easy for users to use the large resources these computers offer.  Without some kind of intelligent job management, some calculations will remain out of reach.  We have made \texttt{mpi\_jm} available in its current state on github\cite{githubJM}.  Its ease of use and the ease with which it can be integrated into an executable lead us to hope it gains widespread adoption, far beyond our immediate usecase.

In our case, unleashing the full potential of these new machines has tantalizing physics implications.
Pushing down the uncertainty on our previous calculation will allow us to compete directly with experiment, and will provide a quantitative bridge between fundamental particle physics and the simplest nuclear observables.
Anchoring these properties in the underlying particle physics will allow us to directly compare precision nuclear experiments to the theory, disentangling effects of known physics from anything beyond our current understanding.

But the potential of these machines is far greater than any one particular nuclear observable.
We expect to attack systems with more than one proton or neutron, measuring their interactions.
Once few-body systems are under control, a quantitative connection to the light nuclei will follow.
This will eliminate the phenomenological input that currently underlies our models of nuclear physics and will provide a complete quantification of the theoretical uncertainty for these light nuclei.
Fitting other many-body methods to these results will propagate this quantification across the periodic table.

One system of enormous interest that may be tractable with LQCD is the three neutron system.  Because they are electrically neutral, it is extraordinarily difficult to build an experiment where three neutrons can interact without any protons.
And yet, this three-neutron interaction is of fundamental interest in nuclear astrophysics and is one of the largest uncertainties in the input to models of compact astrophysical objects like neutron stars.  Gross properties of neutron star interiors will be probed by gravitational wave astronomy, but understanding whether these properties jibe with our theory of nuclear physics will rely on a first-principles theoretical determination of the three-neutron interaction, which can only be achieved with Lattice QCD.  Already in the two-neutron system the tensor contractions take a substantially larger portion of the computing time (closer to 50\%).  The ability to overlay contractions with propagator solves will prove an enormous boon in these more difficult cases.  So, the importance of \texttt{mpi\_jm} to our production will only grow.

Another application of particular interest is the interpretation of dark matter experiments.
Many dark matter experiments are large collections of ultra-pure, very cold, well-isolated and carefully-monitored material.  When a dark matter particle passes through the detector, it may strike a nucleus and result in an observable signal.  Any observation or limit on interaction frequency will be an experimental achievement---but one that tells us first and foremost about how dark matter interacts with large collections of protons and neutrons rather than with the fundamental ingredients of the Standard Model.
Disentangling the nuclear effects from the fundamental effects requires forging a trustable chain of evidence that allows us to translate experimental results into information about new physics.
One part of solving this outstanding theoretical challenge will be precision LQCD nuclear physics calculations.

Similarly, significant resources are being spent on experimental searches for a possible ultra-rare exotic nuclear decay known as \emph{neutrinoless double beta decay} that can help explain why there is more matter than antimatter in our universe.  We recently completed a first calculation of the simplest pieces of this process\cite{Nicholson:2016byl,0vbb-prl} on backfilled and otherwise-wasted time on Titan, but a full understanding of how this process can happen, disentangling known physics from new physics requires additional calculations that will now be possible.

Grounding nuclear physics in the underlying particle physics and eliminating the need for phenomenological input will be a critical step in connecting many modern experiments and observations with new discoveries and frontiers beyond.




==> section/introduction.tex <==
\section{Introduction}

\LaTeX is a system for producing beautiful documents.
It takes as input a set of plain text files, and produces a variety of output types; the most useful to me is PDF.

\git is a decentralized version control system.
It's fantastic.

This repo is an example that is supposed to make it easy to make \git-controlled \LaTeX documents.
In particular, I have written \git hooks that ensure individual commits successfully produce a PDF and ensure that after a pull the PDF is automatically recompiled with the latest edits.
That helps keep everybody\ldots\ on the same page.

I also have a small shell script that reports the status of the repo when the PDF is being compiled that can be immediately incorporated into the \LaTeX document.
The script \texttt{git\_information.sh} produces \texttt{git\_information.tex} which looks, in the current example, like
\begin{verbatim}
% Automatically generated by git_information.sh
\newcommand{\gitRevision}{9c35867408bd1e7915f9f7501ac341fa497834f1}
\newcommand{\gitRevisionDate}{2018-06-08 14:07:44 +0200}
\newcommand{\gitDirtyFiles}{1}
\newcommand{\gitInfo}{\gitDirtyFiles\ files different from commit \gitRevision\ from \gitRevisionDate}
\end{verbatim}
The one dirty file is the one I'm working on---\texttt{section/introduction.tex}.
In \texttt{master.tex}, I have \texttt{\textbackslash include\{git\_information\}} and invoke \texttt{\textbackslash gitInfo} at the end of the abstract, which produces the git status at the bottom of the cover page of this document.

